Thermal and magnetic evolution of an Earth-like planet with a basal magma ocean

Earth's geodynamo has operated for over 3.5 billion years. The magnetic field is currently powered by thermocompositional convection in the outer core, which involves the release of light elements and latent heat as the inner core solidifies. However, since the inner core nucleated no more than 1.5 billion years ago, the early dynamo could not rely on these buoyancy sources. Given recent estimates of the thermal conductivity of the outer core, an alternative mechanism may be required to sustain the geodynamo prior to nucleation of the inner core. One possibility is a silicate dynamo operating in a long-lived basal magma ocean. Here, we investigate the structural, thermal, buoyancy, and magnetic evolution of an Earth-like terrestrial planet. Using modern equations of state and melting curves, we include a time-dependent parameterization of the compositional evolution of an iron-rich basal magma ocean. We combine an internal structure integration of the planet with energy budgets in a coupled core, basal magma ocean, and mantle system. We determine the thermocompositional convective stability of the core and the basal magma ocean, and assess their respective dynamo activity using entropy budgets and magnetic Reynolds numbers. Our conservative nominal model predicts a transient basal magma ocean dynamo followed by a core dynamo after 1 billion years. The model is sensitive to several parameters, including the initial temperature of the core-mantle boundary, the parameterization of mantle convection, the composition of the basal magma ocean, the radiogenic content of the planet, as well as convective velocity and magnetic scaling laws. We use the nominal model to constrain the range of basal magma ocean electrical conductivity and core thermal conductivity that sustain a dynamo.

==> header.tex <==
%=================================================================%
%LATEX DOCUMENT HEADER (Version 03/2022)
%=================================================================%
%=================================================================%
%PACKAGES
%=================================================================%
%Page style
\usepackage{geometry}
\usepackage{fancyhdr}
\usepackage{afterpage}
\usepackage[explicit]{titlesec}
\usepackage{titletoc}
\usepackage{lineno}
%Authors
\usepackage{authblk}
%Bibliography
\usepackage[round]{natbib}
\usepackage{bibentry}
%Fonts
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{libertine}
\usepackage{babel}
\usepackage{textcomp}
\usepackage{contour}
\usepackage[normalem]{ulem}
\usepackage{setspace}
%Lists
\usepackage{enumitem}
\usepackage{etaremune}
%Maths
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage[inter-unit-product=\cdot]{siunitx}
\usepackage{etoolbox}
\usepackage{wasysym}
%Colors
\usepackage[dvipsnames,table]{xcolor}
%Figures
\usepackage{caption}
\usepackage{graphicx}
\usepackage{float}
\usepackage{subfig}
\usepackage{wrapfig}
\usepackage[final]{pdfpages}
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usetikzlibrary{plotmarks}
\usepgfplotslibrary{patchplots}
\usepackage{grffile}
\usepackage[most]{tcolorbox}
\usepackage{rotating}
%Tables
\usepackage{booktabs}
\usepackage{bigstrut}
\usepackage{multirow}
\usepackage{longtable}
\usepackage{tabularx}
%Appendix
\usepackage[header,titletoc,page]{appendix}
%Hyperref
\usepackage{import}
\usepackage{hyperref}
\hypersetup{colorlinks=true,linktoc=all,linkcolor=Black,citecolor=Blue,filecolor=Black,urlcolor=Black}
%Lipsum
\usepackage{lipsum}
%Code
\usepackage{listings}
\lstset{
upquote=true,
columns=flexible,
basicstyle=\ttfamily,
language=[LaTeX]TeX, %langage utilisé
xleftmargin=\dimexpr\fboxsep+\fboxrule,
xrightmargin=\dimexpr\fboxsep+\fboxrule,
texcsstyle=*\color{Maroon}, %couleur des commandes
commentstyle=\color{gray}, % couleur des commentaires
moretexcs={titlecontents,contentslabel,titlerule,contentspage,drh,upDelta}, %mots clés du langage
frame=single,
rulecolor=\color{green!5},
backgroundcolor=\color{green!5}, %couleur de fond
breaklines, %autoriser la césure
numbers=none, %numéros de ligne
frame=r,
framexrightmargin=1pt,
breakindent=1.5em, %longueur d'une tabulation
literate=
{á}{{\'a}}1 {é}{{\'e}}1 {í}{{\'i}}1 {ó}{{\'o}}1 {ú}{{\'u}}1
{Á}{{\'A}}1 {É}{{\'E}}1 {Í}{{\'I}}1 {Ó}{{\'O}}1 {Ú}{{\'U}}1
{à}{{\`a}}1 {è}{{\`e}}1 {ì}{{\`i}}1 {ò}{{\`o}}1 {ù}{{\`u}}1
{À}{{\`A}}1 {É}{{\'E}}1 {Ì}{{\`I}}1 {Ò}{{\`O}}1 {Ù}{{\`U}}1
{ä}{{\"a}}1 {ë}{{\"e}}1 {ï}{{\"i}}1 {ö}{{\"o}}1 {ü}{{\"u}}1
{Ä}{{\"A}}1 {Ë}{{\"E}}1 {Ï}{{\"I}}1 {Ö}{{\"O}}1 {Ü}{{\"U}}1
{â}{{\^a}}1 {ê}{{\^e}}1 {î}{{\^i}}1 {ô}{{\^o}}1 {û}{{\^u}}1
{Â}{{\^A}}1 {Ê}{{\^E}}1 {Î}{{\^I}}1 {Ô}{{\^O}}1 {Û}{{\^U}}1
{œ}{{\oe}}1 {Œ}{{\OE}}1 {æ}{{\ae}}1 {Æ}{{\AE}}1 {ß}{{\ss}}1
{ç}{{\c c}}1 {Ç}{{\c C}}1 {ø}{{\o}}1 {å}{{\r a}}1 {Å}{{\r A}}1
{£}{{\pounds}}1 { ×}{{$\times$}}1,} %correction pour les caractères accentués

%=================================================================%
%ENVIRONMENTS
%=================================================================%
%2 Columns Figures
%=================================================================%
\newenvironment{Figure}
  {\par\medskip\noindent\minipage{\linewidth}}
  {\endminipage\par\medskip}
  
%2 Columns Tables
%=================================================================%
\newenvironment{Table}
  {\par\medskip\noindent\minipage{\linewidth}}
  {\endminipage\par\medskip}

%Homemade track-change: \authorname{remove}{add}
%=================================================================%
\newcommand{\vl}[2]{\textcolor{Red}{\sout{#1}}\textcolor{Red}{\textbf{#2}}}

%Colored answers
%=================================================================%
\newenvironment{ans}{\vspace{4mm}\color{Blue}}{\vspace{4mm}}

%=================================================================%
%PACKAGE OPTIONS
%=================================================================%
%Contour package
%=================================================================%
\contourlength{0.75pt}

%Titlesec package
%=================================================================%
\titleformat{\chapter}[hang]
{\raggedright}
{\parbox[t]{0.15\textwidth}{\filright\fontsize{96pt}{0pt}\selectfont\thechapter}}
{0pt}
{\hfill\Huge\sffamily\parbox[b]{0.85\textwidth}{\filleft #1}} %Chapter format

\titleformat{\part}[hang]
{}
{\filright\LARGE\bfseries\thepart}
{15pt}
{\LARGE\bfseries #1} %Part format

\titlespacing{\part}{0pt}{-20pt}{*2.5}

\titlecontents{part}
[0pt]
{\vspace{10pt}}
{}
{\large\bfseries}
{}
[]

% Captions
%=================================================================%
\captionsetup[table]{labelsep=newline,labelfont=bf}

%Table of content parameters
%=================================================================%
\setcounter{tocdepth}{4}
\setcounter{secnumdepth}{4}  

%=================================================================%
%PAGE STYLE
%=================================================================%
%Geometry
%=================================================================%
\geometry{top=2.5cm,bottom=2.5cm,left=2.5cm,right=2.5cm}

%Colors
%=================================================================%
\definecolor{color1}{gray}{0.6}

%Reduce Bibliography Interligne
%=================================================================%
\setlength{\bibsep}{0.0pt}

%Head and Foot Pages
%=================================================================%
\pagestyle{fancy}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{1pt}
\fancyhf{}
\fancyhead[L]{}
\fancyhead[C]{Evolution of an Earth-like planet with a basal magma ocean}
\fancyhead[R]{}
\fancyfoot[R]{\thepage}
\fancyfoot[C]{}
\fancyfoot[L]{V. Lherm, M. Nakajima, E.G. Blackman}

%Cell color with bookstab
%=================================================================%
\extrarowheight=\aboverulesep
\addtolength{\extrarowheight}{\belowrulesep}
\aboverulesep=0pt
\belowrulesep=0pt

%Section heading
%=================================================================%
\newcommand{\heading}[1]{
    \vspace*{5mm}
    \noindent\textcolor{Black}{\large\bfseries\sffamily #1}\\
    \vspace*{-7mm}\\
    \rule{\linewidth}{1pt}
    \vspace*{-2mm}
}

%=================================================================%
%AUTHOR COORDINATES
%=================================================================%
\newcommand*{\theauthor}[1]{\renewcommand*{\theauthor}{#1}}
\newcommand*{\affiliation}[1]{\renewcommand*{\affiliation}{#1}}
\newcommand*{\department}[1]{\renewcommand*{\department}{#1}}
\newcommand*{\job}[1]{\renewcommand*{\job}{#1}}
\newcommand*{\email}[1]{\renewcommand*{\email}{#1}}
\newcommand*{\addressone}[1]{\renewcommand*{\addressone}{#1}}
\newcommand*{\addresstwo}[1]{\renewcommand*{\addresstwo}{#1}}
\newcommand*{\phonenum}[1]{\renewcommand*{\phone}{#1}}
\newcommand*{\place}[1]{\renewcommand*{\place}{#1}}

%=================================================================%
%MACROS MATHS
%=================================================================%
\newcommand{\Pe}{\mathrm{Pe}}
\newcommand{\Bo}{\mathrm{Bo}}
\newcommand{\Fr}{\mathrm{Fr}}
\newcommand{\Oh}{\mathrm{Oh}}
\newcommand{\We}{\mathrm{We}}
\newcommand{\Sc}{\mathrm{Sc}}
\newcommand{\Ra}{\mathrm{Ra}}
\newcommand{\St}{\mathrm{St}}
\newcommand{\Ro}{\mathrm{Ro}}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\dt}{\mathrm{d}}
\newcommand{\Dt}{\mathrm{D}}
\newcommand{\Ek}{\mathrm{Ek}}
\newcommand{\Le}{\mathrm{Le}}

\renewcommand{\Re}{\mathrm{Re}}
